A Survey of Decomposition-Based Evolutionary Multi-Objective Optimization: Part I-Past and Future

Decomposition has been the mainstream approach in classic mathematical programming for multi-objective optimization and multi-criterion decision-making. However, it was not properly studied in the context of evolutionary multi-objective optimization (EMO) until the development of multi-objective evolutionary algorithm based on decomposition (MOEA/D). In this two-part survey series, we use MOEA/D as the representative of decomposition-based EMO to review the up-to-date development in this area, and systematically and comprehensively analyze its research landscape. In the first part, we present a comprehensive survey of the development of MOEA/D from its origin to the current state-of-the-art approaches. In order to be self-contained, we start with a step-by-step tutorial that aims to help a novice quickly get onto the working mechanism of MOEA/D. Then, selected major developments of MOEA/D are reviewed according to its core design components including weight vector settings, subproblem formulations, selection mechanisms and reproduction operators. Besides, we also overview some selected advanced topics for constraint handling, optimization in dynamic and uncertain environments, computationally expensive objective functions, and preference incorporation. In the final part, we shed some light on emerging directions for future developments.

==> makefile <==
FILE=main

all:	
	latex $(FILE)
	bibtex $(FILE)
	latex $(FILE)
	latex $(FILE)
	dvips -o $(FILE).ps $(FILE).dvi
	ps2pdf $(FILE).ps
	open $(FILE).pdf

clean:
	rm -f *.aux *.blg *.log *.bbl *.out *.bak *.synctex.gz *.synctex.gz\(busy\) *.tex~

cleanall: clean
	rm -f *.dvi $(FILE).ps $(FILE).pdf


==> protocol.tex <==
%!TeX root=main.tex

\section{Protocol for Survey}
\label{sec:protocol}

The workflow of our proposed protocol for carrying out this systematic survey is provided in~\pref{fig:review_protocol}. It consists of three stages, the implementation of which are delineated step by step in the following paragraphs.

\subsection{Search String}
\label{sec:string}

\textcolor{red}{From 16th to 30th December 2022}, we conducted an automatic search over six major scientific literature sources, including \href{https://dl.acm.org/}{\texttt{ACM Library}}, \href{https://ieeexplore.ieee.org/Xplore/home.jsp}{\texttt{IEEE Xplore}}, \href{https://www.sciencedirect.com/}{\texttt{ScienceDirect}}, \href{https://link.springer.com/}{\texttt{SpringerLink}}, \href{https://scholar.google.com/}{\texttt{Google Scholar}} and \href{https://dblp.org/}{\texttt{DBLP}}. According to the functionality of different sources, there are two type of search strings.
\begin{itemize}
    \item For the first five sources, we conduct a full text search where the search string is designed to cover a variety of decomposition-based techniques in the context of MO, EMO, and MCDM. Keywords are properly linked via logical connectors (\texttt{AND}, \texttt{OR}) to build the search term. The final search string is as follows.
        \begin{tcolorbox}[breakable, title after break=, height fixed for = none, colback = red!10!white, boxrule = 0pt, sharpish corners, top = 0pt, bottom = 0pt, left = 1pt, right = 1pt]
            (\lq\lq \texttt{optimization}\rq\rq\ \textcolor{blue}{\texttt{OR}} \lq\lq \texttt{multi-objective}\rq\rq\ \textcolor{blue}{\texttt{OR}} \lq\lq\texttt{evolutionary multi-objective optimization}\rq\rq\ \textcolor{blue}{\texttt{OR}} \lq\lq\texttt{evolutionary computation}\rq\rq\ \textcolor{blue}{\texttt{OR}} \lq\lq\texttt{interactive}\rq\rq\ \textcolor{blue}{\texttt{OR}} \lq\lq\texttt{preference}\rq\rq\ \textcolor{blue}{\texttt{OR}} \lq\lq\texttt{MCDM}\rq\rq) \textcolor{blue}{\texttt{AND}} (\lq\lq\texttt{decomposition}\rq\rq\ \textcolor{blue}{\texttt{OR}} \lq\lq\texttt{reference point}\rq\rq\ \textcolor{blue}{\texttt{OR}} \lq\lq\texttt{scalarizing}\rq\rq\ \textcolor{blue}{\texttt{OR}} \lq\lq\texttt{aggregation}\rq\rq\ \textcolor{blue}{\texttt{OR}} \lq\lq\texttt{MOEA/D}\rq\rq)
        \end{tcolorbox}
        The first set of terms before the \textcolor{blue}{\texttt{AND}} connector consists of the common keywords for research in MO, EMO, and MCDM. In particular, we placed \lq\lq\texttt{interactive}\rq\rq\ and \lq\lq\texttt{preference}\rq\rq\ in the string to cover the emerging preference-based and interactive EMO. The second set of terms mainly focuses on keywords closely related to the decomposition-based techniques and MOEA/D.

    \item In contrast, since the \texttt{DBLP} does not work on the whole search string, we paired each term in the first bracket with each one from the second bracket. The results of all pairs were collected.
\end{itemize}

\subsection{Inclusion, Exclusion, and Cleaning Criteria}
\label{sec:criteria}

For the candidate papers found in the \texttt{Stage 1}, we carry out a housekeeping procedure, according to the dedicated inclusion, exclusion, and cleaning criteria, to constitute the primary studies considered in this survey.

\subsubsection{Inclusion Criteria}
\label{sec:inclusion}

The papers meeting all the following five inclusion criteria are temporarily chosen to constitute the primary studies.
\begin{enumerate}
    \item The study specifies the deign of at least one of the algorithmic components of MOEA/D introduced in~\pref{sec:moead}, including the setting of weight vectors, the subproblem formulation, the mating/environmental selection, and the offspring reproduction.

    \item The study investigates the preference incorporation, interactive EMO, and MCDM in MOEA/D.

    \item The study includes quantitative experimental results with clear insights related to the performance of MOEA/D.

    \item The study includes rigorous analysis toward understanding the theoretical underpinnings of MOEA/D.

    \item The study includes non-trivial applications of MOEA/D and its variants in real-world problems.
\end{enumerate}

\subsubsection{Exclusion Criteria}
\label{sec:exclusion}

Afterwords, the temporarily included studies meeting any of the exclusion criteria below are ruled out from further consideration.
\begin{enumerate}
    \item The study is not highly impactful or visible according to the bibliometric information from Google Scholar\footnote{We admit that the citation count is not the perfect bibliometric to quantify the impact of a paper. Nevertheless, Google Scholar has been used as the major bibilometric source in many studies such as~\cite{FuMS16}.}. Specifically, the threshold is set as $3$ citations per year since its publication. For example, a study published in 2008 is expected to have at least $42$ citations. The only exception is for the work published in the year when we are preparing this article, i.e., 2022. In other words, we consider all publications or pre-prints in \href{https://arxiv.org/}{arXiv} regardless of their citation counts. 

    \item The study is a short or work-in-progress paper, i.e., shorter than 4 pages such as a poster paper published in GECCO Companion.

    \item The study is a trivial application of the vanilla MOEA/D or its established variants.

    \item The study is a review, survey, or tutorial. Note that this type of publication is collectively considered as the source related to the research in MOEA/D.
\end{enumerate}

\begin{remark}
    Note that there is no thumb rule to set the citation threshold. The setting used in this survey is justified from the following two aspects.
    \begin{itemize}
        \item Our aim is to emphasize on the major trends about the further development of MOEA/D as well as the emerging challenges in the EMO community. This is important, as any issue discovered will be particularly prevalent across the most visible studies with even higher impact.

        \item The publication date considered here is the official date that the work appears in the publisher’s webpage assigned with a digital object identifier. Yet, it is not uncommon that many studies are made citable as pre-prints before their actual publication. This has helped to accumulate citations.
    \end{itemize}
\end{remark}

\subsubsection{Cleaning Criteria}
\label{sec:cleaning}

To make sure only significant contributions are analyzed in this survey, we design the following cleaning criteria to further process the primary studies if multiple studies of the same approach are found.
\begin{itemize}
    \item Only the latest version or the extended journal version is considered in the survey.

    \item If the same authors published different studies for the same approach, all studies are retained if they report on different problems.
\end{itemize}

\subsection{Data Analysis}
\label{sec:data_analysis}

\begin{table}[t!]
    \centering
    \caption{Meta features considered in the data collection process.}
    \resizebox{1.0\columnwidth}{!}{ 
    \begin{tabular}{c|c|c}
        \hline
        ID    & Meta feature & RQ(s) \\ \hline\hline
        $I_1$    & Authors & RQ5 \\ \hline
        $I_2$    & Institutions & RQ5 \\ \hline
        $I_3$    & Year & N/A \\ \hline
        $I_4$    & Title & N/A \\ \hline
        $I_5$    & Publication venue (journal or conference) & RQ5 \\ \hline
        $I_6$    & Number of citations & N/A \\ \hline
        $I_7$    & The setting of weight vector & RQ1 \\ \hline
        $I_8$    & Subproblem formulation & RQ1 \\ \hline
        $I_9$    & Mating selection & RQ1 \\ \hline
        $I_{10}$    & Environmental selection & RQ1 \\ \hline
        $I_{11}$   & Reproduction operator & RQ1 \\ \hline
        $I_{12}$   & The type of the targeted problems & RQ2, RQ6 \\ \hline
        $I_{13}$   & Quality indicators for performance assessment & RQ3, RQ6 \\ \hline
        $I_{14}$   & Application domain & RQ4, RQ6 \\ \hline
    \end{tabular}
    }
    \label{tab:meta_feature}
\end{table}

For the primary studies collected in the \texttt{Stage 2}, we design a data analysis protocol to categorize them into different groups that help structure our survey. More specifically, the data analysis protocol is designed based on the $14$ meta features listed in~\pref{tab:meta_feature}.
\begin{itemize}
    \item The first five meta features are used as the identity of the primary studies. In particular, $I_1$, $I_2$, $I_5$ are used in the data mining contributing to the answer of the RQ5.

    \item $I_7$ to $I_{11}$ constitute the major algorithmic components to design a MOEA/D variant as introduced in~\pref{sec:moead}. These help answer the RQ1.

    \item $I_{12}$ helps understand the breadth of MOEA/D and its variants for solving different kinds of MOPs. Besides, it also provides insights about the evolution of research topics in the EMO community and helps identify emerging areas. The relevant information investigated in $I_{12}$ help address both the RQ2 and the RQ6.

    \item $I_{13}$ helps understand the trend of quantitative performance assessment in the EMO community. This provides insights related to both the RQ3 and the RQ6.

    \item $I_{14}$ helps understand the impact of MOEA/D and its variants for solving real-world applications. This contributes to the investigation of the RQ4 and the RQ6.
\end{itemize}

In practice, the data analysis protocol is implemented as the following three-step process.
\begin{enumerate}[Step 1:]
    \item Conduct an initial data analysis to summarize the data and perform a preliminary categorization.

    \item Check the data and categorization to resolve overlaps across more than one categorization.

    \item Eliminate any typo, missing labels, and errors.
\end{enumerate}

\begin{remark}
    There are two cases leading to overlapped categorizations in Step 2.
    \begin{itemize}
        \item First, it is anticipated that more than one of the meta features $I_7$ to $I_{11}$ can be covered in a single paper to design a new algorithm. In this case, we investigate the most influential feature to decide the categorization. Otherwise, further confusions are resolved by consulting the corresponding author(s).

        \item Second, some application papers might not make significant algorithmic contributions. We carefully evaluate the algorithmic contribution(s) with regard to $I_7$ to $I_{11}$ to resolve the potential overlaps.
    \end{itemize}
\end{remark}

\subsection{Overall Results}
\label{sec:protocol_results}

As shown in~\pref{fig:review_protocol}, the \texttt{Stage 1} of our proposed protocol initially obtains a set of \textcolor{red}{$66,786$} studies from various scientific literature sources. Note that duplications are removed by automatically matching their titles\footnote{Patents, citation entries, inaccessible papers, and any other non-English documents are also eliminated.}, leading to a much smaller and more concise set of \textcolor{red}{$4,321$} studies. During the \texttt{Stage 2}, the inclusion criteria is applied to shortlist \textcolor{red}{$1,000$} temporary included studies. Then, they are further compressed according to the exclusion criteria, leading to \textcolor{red}{$500$} candidate studies. A further cleaning process is conducted to rule out different studies that essentially report the same work. Afterwards, only \textcolor{red}{$486$} primary studies are survived for the data analysis conducted in the \texttt{Stage 3}.

